An Analysis of the Search Spaces for Generate and Validate Patch Generation Systems

We present the first systematic analysis of the characteristics of patch search spaces for automatic patch generation systems. We analyze the search spaces of two current state-of-the-art systems, SPR and Prophet, with 16 different search space configurations. Our results are derived from an analysis of 1104 different search spaces and 768 patch generation executions. Together these experiments consumed over 9000 hours of CPU time on Amazon EC2. The analysis shows that 1) correct patches are sparse in the search spaces (typically at most one correct patch per search space per defect), 2) incorrect patches that nevertheless pass all of the test cases in the validation test suite are typically orders of magnitude more abundant, and 3) leveraging information other than the test suite is therefore critical for enabling the system to successfully isolate correct patches. We also characterize a key tradeoff in the structure of the search spaces. Larger and richer search spaces that contain correct patches for more defects can actually cause systems to find fewer, not more, correct patches. We identify two reasons for this phenomenon: 1) increased validation times because of the presence of more candidate patches and 2) more incorrect patches that pass the test suite and block the discovery of correct patches. These fundamental properties, which are all characterized for the first time in this paper, help explain why past systems often fail to generate correct patches and help identify challenges, opportunities, and productive future directions for the field.

==> design.tex <==
\section{Design}
\label{sec:design}

SPR starts with a program with a defect and a test suite. The suite contains 
{\em positive test cases}, for
which the program already produces correct outputs, and {\em negative test
cases}, which expose the defect that causes the program to produce incorrect
outputs. The goal is to generate a repair that enables the program to
pass the supplied test suite (i.e, produce correct outputs for all test cases
in the test suite).

SPR first uses fault localization to identify target
statements to transform~\cite{FaultLocalization, Jose:2011, AngelicDebugging}. 
It then stages the search for a successful repair as follows. 
It first selects a transformation schema to apply to a target statement. The result is a
candidate repair template, which may contain an abstract expression as the 
template parameter. {\name} then uses target value search to determine
if there is any parameter value that would instantiate the candidate repair template
to deliver a successful repair. If so, SPR synthesizes candidate parameter values
and attempts to validate each resulting repair in turn. 

\if 0
Section~\ref{sec:overview} presents an overview
the SPR patch generation system. Section~\ref{sec:design:core} presents
a simple imperative core language that we use to illustrate 
the key concepts in the {\name} repair algorithm. Section~\ref{sec:design:schemas} presents the
transformation schemas as they apply to the core language. Section~\ref{sec:design:algo} 
presents the core repair algorithm, including condition synthesis. Section~\ref{sec:design:extensions} 
discusses how we extend the core algorithm to handle C. 

\subsection{Overview} 
\label{sec:overview}

% SPR is a generate-and-validate program repair system~\cite{ClearView}.
SPR starts with a program with a defect and a test suite. The suite contains 
{\em positive test cases}, for
which the program already produces correct outputs, and {\em negative test
cases}, which expose the defect that causes the program to produce incorrect
outputs. The goal is to generate a patch that enables the program to
pass the supplied test suite (i.e, produce correct outputs for all test cases
in the test suite).

SPR first uses fault localization to identify target
statements to transform~\cite{FaultLocalization, Jose:2011, AngelicDebugging}. 
It then stages the search for
a successful patch as follows. It first selects a
transformation schema to apply to a target statement. The result is a
{\em candidate repair template}, which may contain an abstract expression as the 
template parameter. {\name} then uses target value search to determine
if there is any parameter value that would instantiate the candidate repair template
to deliver a successful patch. If so, SPR synthesizes candidate parameter values
and attempts to validate each resulting patch in turn. 

\comment{
The search space 
(which is generated by the transformation schemas) and the search algorithm
(which is 

 the repair template to determine whether any concrete repair
instantiated from the template can pass the supplied test cases. 

If so, at the
second stage {\name} generates and validates each concrete repair instantiated
from the validated template.


SPR uses a set of parameterized transformation schemas to generate a search
space of patches.  After using fault localization to identify target
statements to transform~\cite{FaultLocalization}, SPR first selects a
transformation schema to apply to a target statement. The result is a
{\em repair template}, which may 
generate a candidate repair template, which may
contain an abstract expression as the template parameter. {\name} then
validates the repair template to determine whether any concrete repair
instantiated from the template can pass the supplied test cases. If so, at the
second stage {\name} generates and validates each concrete repair instantiated
from the validated template.

Generate-and-validate systems operate on a search
space of candidate patches and explore the space with a search algorithm to
validate each candidate patch.  ystems typically use
defect localization algorithms to identify target statements that may
be responsible for or related to the defect~\cite{FaultLocalization}, then 
generate patches that transform the target statement. 
When it finds a patch that passes the test
suite, the system accepts the patch.  The design of the search space and search
algorithm are clearly critical for the success of the technique.

We present a new program repair system, {\name}, that uses a novel {\em staged
repair} strategy to generate and efficiently explore a rich and structured
space of candidate repairs. 


The advantage of introducing repair templates to stage the repair process is
that it enables {\name} to efficiently discard those repairs that cannot pass
the supplied test suite. The abstract expression in each repair template, once
instantiated, could generate many concrete repairs. {\name} does not attempt to
validate these concrete repairs, if the template fails the validation at the
first stage.

\subsection{Condition Synthesis}
}
Many useful patches manipulate branch conditions. {\name} works with the following
transformation schemas to generate repair templates for such patches.
\begin{itemize} % \itemsep 0pt \parskip 0pt
\item {\bf Condition Refinement:} Given a target if statement, {\name} transforms the
condition of the if statement by conjoining or disjoining an abstract condition to the 
original if condition. 
\item {\bf Condition Introduction:} Given a target statement, {\name} transforms
the program so that the statement executes only if an abstract condition is true. 
\item {\bf Conditional Control Flow Introduction:} {\name} inserts a new 
control flow statement (return, break, or goto an existing label) that executes
only if an abstract condition is true.
\end{itemize}

To realize the staged repair strategy on the generated templates from these
transformation schemas, {\name} uses a novel {\em condition synthesis}
technique. For each of the templates, {\name} stages the condition synthesis as
follows. It first finds target values for the condition 
that deliver correct results on all
test cases in the test suite. It then generates a logical expression that
successfully approximates these target values:
\begin{itemize} % \itemsep 0pt \parskip 0pt
\item {\bf Semantics-Preserving Target Conditions:} The abstract condition of each 
template has a target condition value
that preserves the semantics of the program. 
For Condition Transformation, the semantics-preserving value
is true for conjoined conditions and false for disjoined conditions. 
For Condition Introduction, the semantics-preserving value is true (so that the target statement always executes).
For Conditional Control-Flow Introduction, the semantics-preserving value 
is false (so that the introduced control flow statement never executes). 

\item {\bf Target Condition Value Search:} 
%{\name} applies the schema to the program, using an abstract target
%condition for the parameter. 
{\name} applies the template and 
repeatedly reexecutes the
transformed program with the abstract condition on the negative test cases. On each execution it
generates a sequence of 0/1 values for the abstract condition
(the sequence contains one value for each execution of the abstract condition). 
The goal is to find sequences of target condition values that produce
correct outputs for all negative test cases. 

\item {\bf Record Mappings:} 
{\name} executes instrumented versions of the program on both negative and positive test cases. 
For each negative test case, it uses the discovered target condition values
that produce the correct output. For each positive test case, it uses the 
semantics-preserving target condition values. 
For each execution of the abstract target condition, the instrumentation records a mapping from
the values of variables in the surrounding context to the corresponding target condition value. 

\item {\bf Condition Generation:} 
The goal is to obtain a logical expresssion, over the variables in the
surrounding context, that generates the same target condition values as those
recorded in the successful instrumented executions. In practice, when a correct
repair exists in the search space, it is almost always possible to realize this
goal. In general, however, a correct repair may not need to exactly match the
target condition values~\cite{Wang:2003}. {\name} therefore does not require an
exact match --- it works with the recorded mappings to generate symbolic
conditions that maximize the number of generated target condition values that
are the same as the target condition values recorded in the previous
instrumented executions (in many but not all cases these logical expressions
match all of the recorded target condition values). 

\item {\bf Condition Test:} 
{\name} instantiates the template with the generated condition, generates the
concrete repair, and runs the repaired program to determine if the program
produces correct outputs for all test cases.  If not, {\name} proceeds on to
test the next generated condition in the sequence. 
\end{itemize}

Staged repair and condition synthesis 
significantly reduce the number of candidate repairs that {\name} attempts 
to validate and therefore enable {\name} to efficiently explore its search space. 
In practice, well over 99\% of the candidate repair templates are rejected in 
the first stage (when the target value search fails to find values 
that produce correct results), eliminating the need to 
consider any patch at all  
for the overwhelming majority of templates. 
%And when the target
%value search succeeds, the resulting values enable SPR to quickly find conditions that are likely to 
%deliver a successful repair. 

In addition to the condition-oriented schemas, {\name} also
deploys several schemas that focus on changing the values 
of target program variables.
\begin{itemize} % \itemsep 0pt \parskip 0pt 
\item \textbf{Insert Initialization: } For each identified
statement, {\name} generates repairs that insert a memory initialization 
statement before the identified statement.

\item \textbf{Value Replacement: } For each identified statement, {\name}
generates repairs that replace either 1) one variable with another, 2)
an invoked function with another, or 3) a constant
with another constant. 

\item \textbf{Copy and Replace: } For each identified statement, {\name}
generates repairs that copy an existing statement to the program point
before the identified statement and then apply a Value Replacement
transformation. 
\end{itemize}
The rationale for the Copy and Replace modification is to exploit redundancy in
the program --- some successful repairs can be constructed from
code that already exists in the program~\cite{Barr:2014}. The goal of the
Replace part of Copy and Replace is to obtain a rich repair search space that
includes variable replacement to enable copied code to operate successfully in
a new naming context. The success of these modifications  is consistent with
previous work that shows that, without replacement, only approximately 10\% of
developer changes can be fully derived from existing statements without
modification~\cite{Martinez:2014, Barr:2014, Gabel:2010}. 
\comment{This fact may also
provide insight into the poor performance of previous patch generation
systems~\cite{LeGoues:2012, Weimer:2013, Qi:2014} (which only copy statements without
expression-level modifications). 
}
\fi

\begin{figure}
\small
\begin{Verbatim}[commandchars=\\\{\}, codes={\catcode`$=3\catcode`_=8}]
$c$ := 1 $\mid$ 0 $\mid$ $c_1$ && $c_2$ $\mid$ $c_1$ || $c_2$ $\mid$ !$c_1$ $\mid$ $(c_1)$ $\mid$ $v$==$\mathit{const}$
$\mathit{prts}$ := print $v$ $\mid$ print $\mathit{const}$ 
$\mathit{simps}$ := $v$ = $v_1$ op $v_2$ $\mid$ $v$ = $\mathit{const}$ $\mid$ $v$ = read $\mid$ $\mathit{prts}$
$\mathit{ifs}$    := if ($c$) $\ell_1$ $\ell_2$
$\mathit{absts}$ \hspace{1.2mm}:= if ($c$ && !abstc) $\ell_1$ $\ell_2$ $\mid$ if ($c$ || abstc) $\ell_1$ $\ell_2$
         $\mid$ print abstval
$s$     \hspace{0.6mm}:= skip $\mid$ stop $\mid$ $\mathit{simps}$ $\mid$ $\mathit{ifs}$ $\mid$ $\mathit{absts}$ 
$v, v_1, v_2 \in \text{Variable}$  $const \in \text{Int}$  $\ell_1, \ell_2 \in \text{Label}$ 
$c, c_1, c_2 \in \text{CondExpr}$  $s \in \text{Stmt}$    $\mathit{ifs} \in \text{IfStmt}$
$\mathit{prts} \in \text{PrintStmt}$    $\mathit{simps} \in \text{SimpleStmt}$
$\mathit{absts} \in \text{AbstStmt}$
\end{Verbatim}
\vspace{-3mm}
\caption{The language statement syntax}
\label{fig:lang}
\vspace{-4mm}
\end{figure}

\begin{figure*}[t!]
\scriptsize
\input{figs/semantics-merged.tex}
\caption{Small step operational semantics}
\label{fig:semantic}
\label{fig:semantic-abstc}
\end{figure*}

\subsection{Core Language}
\label{sec:design:core}

\noindent \textbf{Language Syntax: }
Figure~\ref{fig:lang} presents the syntax of the core language that we use to
present our algorithm. The current implementation of {\name} works with
applications written in the C programming language. See
Section~\ref{sec:design:extensions} for the extension of our algorithm to
handle C. 

A program is a pair $\langle p, n \rangle$, where $p: \text{Label} \to
\text{Statement}$ maps each label to the corresponding statement and $n:
\text{Label} \to \text{Label}$ maps each label to the label of the next
statement to execute. $\ell_0$ is the label of the first statement in the
program. 

The language in Figure~\ref{fig:lang} contains arithmetic statements and if
statements. An if statement of the form ``\texttt{if ($c$) $\ell_1$ $\ell_2$}''
transfers the execution to $\ell_1$ if $c$ is 1 and
$\ell_2$ if $c$ is 0. The language uses if statements to encode loops. 
A statement of the form ``\texttt{$v$ = read}'' reads an integer
value from the input and stores the value to the variable $v$. A statement of
the form ``\texttt{print $v$}'' prints the value of the variable $v$ to the
output. Statements that contain an abstract expression (i.e.,
\texttt{AbstStmt}) are temporary statements that the algorithm may introduce
into a program during the repair algorithm. Such statements do not 
appear in the original or repaired programs.

\begin{figure*}
\small
\begin{displaymath}
\begin{array}{lll}
\mathrm{M}(\langle p, n \rangle) & = & \mathrm{M_{\text{IfStmt}}}(\langle p, n \rangle) \cup \mathrm{M_{\text{Stmt}}}(\langle p, n \rangle) \\

\mathrm{M_\text{IfStmt}}(\langle p, n \rangle) & = & \cup_{\ell \in \mathit{TL}(\langle p, n \rangle), p(\ell) \in \text{IfStmt}} (\mathrm{M_{\text{Tighten}}}(\langle p, n \rangle, \ell) \cup \mathrm{M_{\text{Loosen}}}(\langle p, n \rangle, \ell))\\

\mathrm{M_\text{Stmt}}(\langle p, n \rangle) & = &
\cup_{\ell \in \mathit{TL}(\langle p, n \rangle)}(\mathrm{M_{\text{Control}}}(\langle p, n \rangle, \ell) \cup \mathrm{M_{\text{Init}}}(\langle p, n \rangle, \ell ) \cup \mathrm{M_{\text{Guard}}}(\langle p, n \rangle, \ell) \cup 
\mathrm{M_{\text{Rep}}}(\langle p, n \rangle, \ell) \cup \mathrm{M_{\text{CpRep}}}(\langle p, n \rangle, \ell))\\

\mathrm{M_{\text{Tighten}}}(\langle p, n \rangle, \ell) & = & \{\langle p[\ell \mapsto \text{if $(c \texttt{ \&\& } \texttt{!abstc})$ $\ell_1$ $\ell_2$} ], n \rangle \} \text{, where } p(\ell) = \text{if $(c)$ $\ell_1$ $\ell_2$} \\
\mathrm{M_{\text{Loosen}}}(\langle p, n \rangle, \ell) & = & \{\langle p[\ell \mapsto \text{if $(c \texttt{ || } \texttt{abstc})$ $\ell_1$ $\ell_2$} ], n \rangle \} \text{, where } p(\ell) = \text{if $(c)$ $\ell_1$ $\ell_2$} \\
\mathrm{M_{\text{Control}}}(\langle p, n \rangle, \ell) & = & 
\{ \langle p[\ell\prime \mapsto p(\ell)][\ell\prime\prime \mapsto \texttt{stop}][\ell \mapsto \text{if $($0$ \texttt{ || } \texttt{abstc})$ $\ell\prime\prime$ $n(\ell)$}], 
n[\ell\prime \mapsto n(\ell)][\ell \mapsto \ell\prime][\ell\prime\prime \mapsto \ell\prime] \rangle \} \\
\mathrm{M_{\text{Guard}}}(\langle p, n \rangle, \ell) & = & \{\langle p[\ell\prime \mapsto p(\ell)][\ell \mapsto \texttt{if $($1$ \texttt{ \&\& }\texttt{!abstc})$ $\ell\prime$ $n(\ell)$}], n[\ell\prime \mapsto n(\ell)] \rangle \} \\
\mathrm{M_{\text{Init}}}(\langle p, n \rangle, \ell) & = & \{\langle p[\ell\prime \mapsto p(\ell)][\ell \mapsto \texttt{$v$ = $0$}], n[\ell\prime \mapsto n(\ell)][\ell \mapsto \ell\prime] \rangle \mid \forall v \in \mathit{Vars}(p(\ell)) \} \\
\mathrm{M_{\text{Rep}}}(\langle p, n \rangle, \ell) & = & \{\langle p[\ell \mapsto s], n \rangle \mid s \in \mathrm{RepS}(p, p(\ell)) \} \\
\mathrm{M_{\text{CpRep}}}(\langle p, n \rangle, \ell) & = & \{\langle p[\ell\prime \mapsto p(\ell)][\ell \mapsto s], n[\ell\prime \mapsto n(\ell)][\ell \mapsto \ell\prime] \rangle, \\
& & \, \, \, \langle p[\ell\prime \mapsto p(\ell)][\ell \mapsto s\prime)], n[\ell\prime \mapsto n(\ell)][\ell \mapsto \ell\prime] \rangle \mid \forall s \in \mathit{SimpleS}(\langle p, n \rangle), \, \forall s\prime \in \mathrm{RepS(p, s)} \} \\ 
\mathrm{RepS}(p, \texttt{$v$ = $v_1$ op $v_2$}) & = & \{\texttt{$v\prime$ = $v_1$ op $v_2$}, \texttt{$v$ = $v\prime$ op $v_2$}, \texttt{$v$ = $v_1$ op $v\prime$} \mid \forall v\prime \in \mathit{Vars}(p)\} \\
\mathrm{RepS}(p, \texttt{$v$ = $\mathit{const}$}) & = & \{\texttt{$v\prime$ = $\mathit{const}$}, \texttt{$v$ = $\mathit{const}\prime$} \mid \forall v\prime \in \mathit{Vars}(p), \, \forall \mathit{const}\prime \in \mathit{Consts}(p)\} \\
\mathrm{RepS}(p, \texttt{$v$ = read}) & = & \{\texttt{$v\prime$ = read} \mid \forall v\prime \in \mathit{Vars}(p)\} \\
\mathrm{RepS}(p, \mathit{prts}) & = & \{\texttt{print abstval} \}, \text{where $\mathit{prts} \in \texttt{PrintStmt}$}  \\ %\{\texttt{print $v\prime$} \mid \forall v\prime \in \mathit{Vars}(p)\} \\
\mathrm{RepS}(p, s) & = & \emptyset, \text{ where } s \notin \texttt{SimpleStmt}
\end{array}
\vspace{-4mm}
\end{displaymath}
\caption{The program transformation function $\mathrm{M}$. Note that $\ell\prime$ and $\ell\prime\prime$ are fresh labels.}
\label{fig:transform}
\vspace{-4mm}
\end{figure*}

\sloppypar{
\noindent \textbf{Program State:}
A program state $\langle \ell, \sigma, I, O, D, R, S \rangle$ contains 
the current program point (a label $\ell$), the current environment that maps
each variable to its value ($\sigma : \text{Variable}\to\text{Int}$), the
remaining input ($I$), and the generated output ($O$). 
$I$ is a sequence of integer values (i.e.,
$\mathop{\text{Sequence}}(\text{Int})$).
$O$ is a sequence of integer and abstract values (i.e.,
$\mathop{\text{Sequence}}(\text{Int} \cup \{\texttt{abstval}\})$).

To support the
extension to programs with abstract expressions, the program state 
also contains a sequence of future
abstract condition values ($D$), a sequence of recorded abstract condition
values ($R$), and a sequence of recorded environments for each abstract
expression execution ($S$). 
$D$ and $R$ are sequences of zero or
one values (i.e., $\mathop{\text{Sequence}}(0 \mid 1)$). $S$ is a sequence of
environments (i.e.,
$\mathop{\text{Sequence}}(\text{Variable}\to\text{Int})$). 

The first three rules in Figure~\ref{fig:semantic} present the operational semantics of 
input read, if, and print statements.
``$\circ$'' in Figure~\ref{fig:semantic} is
the sequence concatenation operator.
The notation ``$\sigma \vdash c
\Rightarrow x$'' indicates that the condition $c$ evaluates to $x$ under the
environment $\sigma$.  
Note that for programs that do not contain abstract expressions, 
$D$, $R$, and $S$ are unchanged.
See our technical report~\cite{SPRTechReport} for the rules for other
kinds of statements.
%Our technical 
%report presents a (standard) operational semantics, which
%leaves $D$, $R$, and $S$ unchanged for programs that do not contain
%abstract conditions~\cite{SPRTechReport}. 
}

%Figure~\ref{fig:semantic} presents the small step operational semantics of our
%language for statements without abstract conditions. ``$\circ$'' in
%Figure~\ref{fig:semantic} is the sequence concatenation operator. The notation
%``$\sigma \vdash c \Rightarrow x$'' indicates that the condition $c$ evaluates
%to $x$ under the environment $\sigma$.  
%$D$, $R$, and $S$ are unchanged in these rules because these statements
%do not contain an abstract condition.

\subsection{Transformation Schemas}
\label{sec:design:schemas}

Figure~\ref{fig:transform} presents our program transformation function
$\mathrm{M}$. It takes a program $\langle p, n \rangle$ and produces a set of
candidate modified programs after transformation schema application. 
$\mathit{TL}(\langle p, n \rangle)$
is the set of target statement labels to transform. Our 
error localizer (Section~\ref{sec:design:extensions}) 
identifies this set of statements. 
$\mathit{SimpleS}(p)$ denotes all simple statements (i.e. \texttt{SimpleStmt})
in $p$. $\mathit{Vars}(p)$ and $\mathit{Vars}(s)$ denote all variables in the
program $p$ and in the statement $s$, respectively. $\mathit{Consts}(p)$ denotes all constants in $p$.
$\mathrm{RepS}(p, s)$ is an utility function that returns the set of statements
generated by replacing a variable or a constant in $s$ with other variables or
constants in $p$.
Specifically, {\name} works with the following transformation schemas:
\begin{itemize} % \itemsep 0pt \parskip 0pt
\item {\bf Condition Refinement:} Given a target if statement, {\name} transforms the
condition of the if statement by conjoining or disjoining an abstract condition to the 
original if condition ($\mathrm{M_{\text{Tighten}}}$ and $\mathrm{M_{\text{Loosen}}}$).

\item {\bf Condition Introduction:} Given a target statement, {\name} transforms
the program so that the statement executes only if an abstract condition is true ($\mathrm{M_{\text{Guard}}}$). 

\item {\bf Conditional Control Flow Introduction:} {\name} inserts a new 
control flow statement (return, break, or goto an existing label) that executes
only if an abstract condition is true ($\mathrm{M_{\text{Control}}}$).

\item \textbf{Insert Initialization: } For each identified
statement, {\name} generates repairs that insert a memory initialization 
statement before the identified statement ($\mathrm{M_{\text{Init}}}$).

\item \textbf{Value Replacement: } For each identified statement, {\name}
generates repairs that replace either 1) one variable with another, 2)
an invoked function with another, or 3) a constant
with another constant ($\mathrm{M_{\text{Rep}}}$). 

\item \textbf{Copy and Replace: } For each identified statement, {\name}
generates repairs that copy an existing statement to the program point
before the identified statement and then apply a Value Replacement
transformation ($\mathrm{M_{\text{CpRep}}}$). 
\end{itemize}

Note that the transformation schemas $\mathrm{M_{\text{Tighten}}}$,
$\mathrm{M_{\text{Loosen}}}$, $\mathrm{M_{\text{Guard}}}$, and
$\mathrm{M_{\text{Control}}}$ introduce an abstract condition into the 
generated candidate programs. The transformation schemas $\mathrm{M_{\text{Rep}}}$
and $\mathrm{M_{\text{CpRep}}}$ may introduce a print statement with an abstract
expression. These abstract conditions and expressions will be handled by the repair
algorithm later.

\if 0
The transformation function in Figure~\ref{fig:transform} applies condition
refinement schemas ($\mathrm{M_{\text{Tighten}}}$,
$\mathrm{M_{\text{Loosen}}}$) to all target if statements. It applies the
condition introduction schema ($\mathrm{M_{\text{Guard}}}$) and conditional
control flow introduction schema ($\mathrm{M_{\text{Control}}}$) to all target
statements. These four schemas introduce an abstract condition into the
generated candidate programs that will be handled by condition synthesis.

The transformation function also applies the insert initialization schema
($\mathrm{M_{\text{Init}}}$), value replacement schema
($\mathrm{M_{\text{Rep}}}$), and copy and replace schema
($\mathrm{M_{\text{CpRep}}}$) to all target statements. Note that
$\mathrm{RepS}(p, s)$ is an utility function that returns the set of statements
generated by replacing a variable or a constant in $s$ with other variables or
constants in $p$. The latter two schemas may introduce a print statement with 
an abstract expression which will be handled by the staged repair algorithm.
\fi

\subsection{Staged Repair with Condition Synthesis}
\label{sec:design:algo}

Figure~\ref{fig:repair} presents our main staged repair algorithm with
condition synthesis. Given a program $\langle p, n \rangle$, a set of positive
test cases $\mathit{PosT}$, and a set of negative test cases $\mathit{NegT}$,
the algorithm produces a repaired program $\langle p\prime, n\prime \rangle$
that passes all test cases. $\mathrm{Exec}(\langle p, n \rangle, I, D)$ at
lines 6, 13, 21, and 37 produces the results of running the program $\langle p, n
\rangle$ on the input $I$ given the future abstract condition value sequence
$D$. $\mathrm{Test}(\langle p, n \rangle, \mathit{NegT}, \mathit{PosT})$ at
lines 31, 40, and 42 produces a boolean to indicate whether the program $\langle p,
n \rangle$ passes all test cases. See Figure~\ref{fig:exec-test-flip-f}
for the definitions of $\mathrm{Exec}$ and $\mathrm{Test}$.

The algorithm enumerates all transformed candidate programs in the search space
derived from our transformation function $\mathrm{M}(\langle p, n \rangle)$
(line 1). If the candidate program does not contain an abstract expression, the
algorithm simply uses $\mathrm{Test}$ to validate the program
(lines 42-43). If the candidate program contains an abstract condition, the
algorithm applies condition synthesis (lines 3-33) in two stages, target condition
value search and condition generation.

\noindent \textbf{Target Condition Value Search:}
We augment the operational semantics of the core language to handle statements
with an abstract condition. The last four rules in
Figure~\ref{fig:semantic-abstc} present the semantics of ``\texttt{if ($c$ \&\&
abstc) $\ell_1$ $\ell_2$}''. The rules for ``\texttt{if ($c$ || abstc) $\ell_1$
$\ell_2$}'' are similar~\cite{SPRTechReport}. 

The fifth rule in Figure~\ref{fig:semantic-abstc} specifies the case where the
result of the condition does not depend on the abstract condition (the
semantics implements short-circuit conditionals).  In this case the execution
is transfered to the corresponding labels with $D$, $R$, and $S$ unchanged. The
sixth rule specifies the case where there are no more future abstract condition
values in $D$ for the abstract condition \texttt{abstc}. This rule uses the
semantics-preserving value for the abstract condition \texttt{abstc}, with $R$
and $S$ appropriately updated. The last two rules specify the case where $D$ is
not empty. In this case the execution continues as if the abstract condition
returns the next value in the sequence $D$, with $R$ and $S$ updated
accordingly.

\if 0
\begin{figure*}
\scriptsize
\input{figs/semantics-abstc.tex}
\caption{Small step operational semantics for if statements with abstract condition}
\label{fig:semantic-abstc}
\vspace{-4mm}
\end{figure*}
\fi

For each negative test case, the algorithm in Figure~\ref{fig:repair} searches
a sequence of abstract condition values with the goal of finding a sequence of
values that generates the correct output for the test case (lines 5-19).
$\mathrm{Flip}$ is an utility function that flips the last non-zero value in a
given value sequence (see Figure~\ref{fig:exec-test-flip-f} for the formal
definition). The algorithm (line 13) executes the program with different future
abstract condition value sequences $D$ to search for a sequence that passes
each negative test case. If the algorithm cannot find such a sequence,
it moves on to the next candidate program (line 16).

Note that the program may execute an abstract condition multiple times.
{\name} tries a configurable number (in our current implementation, 11) 
of different abstract condition value sequences for each negative
test case in the loop (lines 8-14).
At each iteration (except the last) of the
loop, the algorithm flips the last non-zero value in the previous
sequence. In the last iteration {\name} flips all
abstract condition values to one (line 10 in Figure~\ref{fig:repair}). 

The rationale is that, in practice, if a negative test case
exposes an error at an if statement, either the last few executions 
of the if statement or all of the executions take the wrong branch
direction. This empirical property holds for all defects in our
benchmark set. 

If a future abstract condition value sequence can be found for every negative
test case, the algorithm concatenates the found sequences $R\prime$ and the
corresponding recorded environments to $S\prime$ (lines 18-19). It
then executes the candidate program with the positive test cases and concatenates
the sequences and the recorded environments as well (lines 22-23). Note that
for positive cases the algorithm simply returns zero for all abstract
conditions, so that the candidate program has the same execution as the
original program.

\begin{figure*}[t!]
\scriptsize
\begin{mathpar}
\begin{array}{l}
\mathrm{Exec}(\langle p, n \rangle, I, D) = \\
\left\{  
\begin{array}{ll}
\langle O, R, S \rangle & \exists I\prime, O, R, S, \text{such that } \langle \ell_0, \sigma_0, I, \epsilon, D, \epsilon, \epsilon \rangle  \execute{\langle p, n \rangle} \\
& \langle \texttt{nil}, \sigma, I\prime, O, D\prime, R, S \rangle \\
\bot & \text{otherwise}
\end{array}
\right. 
\\
\end{array}
\begin{array}{l}
\mathrm{Test}(\langle p, n \rangle, \mathit{NegT}, \mathit{PosT}) = \\
\left\{
\begin{array}{ll}
\texttt{False} & \exists \langle I, O \rangle \in (\mathit{NegT} \cup \mathit{PosT}), \text{such that } \\
& \mathrm{Exec}(\langle p, n \rangle, I, \epsilon) = \langle O\prime, R, S \rangle, \, O \neq O\prime \\
\texttt{True} & otherwise
\end{array}
\right.\\
\end{array}
\and 
\inferrule
{}
{F(\epsilon, \epsilon, c) = 0} \and
\inferrule
{\sigma \vdash c \Rightarrow x }
{F(x \circ R, \sigma \circ S, c) = F(R, S, c) + 1} \and
\inferrule
{\sigma \vdash c \Rightarrow (1-x)}
{F(x \circ R, \sigma \circ S, c) = F(R, S, c)} \and
\inferrule
{}
{\mathrm{Flip}(\epsilon) = \epsilon} \and
\inferrule
{R = R\prime \circ 0}
{\mathrm{Flip}(R) = R\prime \circ 1} \and
\inferrule
{R = R\prime \circ 1}
{\mathrm{Flip}(R) = \mathrm{Flip}(R\prime)}
\and 
\\
V(\epsilon, \epsilon, S, C) = C \and
\inferrule
{O\prime \neq O \\ O\prime = \epsilon \text{ or } O = \epsilon}
{V(O\prime, O, S, C) = \emptyset}
\and
\inferrule
{S=\sigma \circ S_0 \\ O\prime = x \circ O_0\prime \\ O = y \circ O_0 \\ x = y }
{V(O\prime, O, S, C) = V(O_0\prime, O_0, S_0, C)}
\and
\inferrule
{O\prime = x \circ O_0\prime \\ O = y \circ O_0 \\ x \neq y \\ x \neq \texttt{abstval}}
{V(O\prime, O, S, C) = \emptyset }
\and
\inferrule
{S=\sigma \circ S_0 \\ O\prime = \texttt{abstval} \circ O_0\prime \\ O = y \circ O_0 \\ C\prime = V(O_0\prime, O_0, S_0, C)}
{V(O\prime, O, S, C) = \{ v \mid \sigma(v)=y, v \in C\prime \} \cup \{y \mid y \in C\prime\}}
\end{mathpar}
\caption{Definitions of $\mathrm{Exec}$, $\mathrm{Test}$, $\mathrm{Flip}$, $\mathrm{F}$, and $\mathrm{V}$ }
\label{fig:exec-test-flip-f}
\end{figure*}

\begin{algorithm}
\scriptsize
\SetNlSty{}{}{}
\DontPrintSemicolon
\SetKw{In}{ in }
\SetKw{And}{ and }
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{original program $\langle p, n \rangle$}
\Input{positive and negative test cases $\mathit{NegT}$ and $\mathit{PosT}$, each is a set of pairs $\langle I, O \rangle$ where $I$ is the test input and $O$ is the expected output.}
\Output{the repaired program $\langle p\prime, n\prime \rangle$, or $\emptyset$ if failed}
\For {$\langle p\prime, n\prime \rangle$ \In $M(\langle p, n \rangle)$}{
 \If {$p\prime$ contains \texttt{abstc}} {
   $R\prime \longleftarrow \epsilon$\;
   $S\prime \longleftarrow \epsilon$\;
   \For {$\langle I, O \rangle$ \In $\mathit{NegT}$} {
     $\langle O\prime, R, S \rangle \longleftarrow \mathrm{Exec}(\langle p\prime, n\prime \rangle, I, \epsilon)$\;
     $\mathit{cnt} \longleftarrow 0$\;
     \While {$O\prime \neq O$ \And $\mathit{cnt} \leq 10$} {
       \If {$\mathit{cnt} = 10$} {
         $D \longleftarrow 1\circ1\circ1\circ1\cdots$
       }
       \Else {
         $D \longleftarrow \mathrm{Flip}(R)$
       }
       $\langle O\prime, R, S \rangle \longleftarrow \mathrm{Exec}(\langle p\prime, n\prime \rangle, I, D)$\;
       $\mathit{cnt} \longleftarrow \mathit{cnt} + 1$\;
     }
     \If {$O \neq O\prime$} {
       \text{skip to the next candidate $\langle p\prime, n\prime \rangle$}
     }
     \Else {
       $R\prime \longleftarrow R\prime \circ R$\;
       $S\prime \longleftarrow S\prime \circ S$\;
     }
   }
   \For {$\langle I, O \rangle$ \In $\mathit{PosT}$} {
     $\langle O\prime, R, S \rangle \longleftarrow \mathrm{Exec}(\langle p\prime, n\prime \rangle, I, \epsilon)$ \;
     $R\prime \longleftarrow R\prime \circ R$\;
     $S\prime \longleftarrow S\prime \circ S$\;
   }
%   $C \longleftarrow \mathrm{GenConds}(R\prime, S\prime)$\;
   $C \longleftarrow \{ \}$\;
   \For {$\sigma \In S\prime$} {
     $C \longleftarrow C \cup \{ \texttt{($v$ == $\mathit{const}$)}, \texttt{!($v$ == $\mathit{const}$)} \mid  \forall v \forall \mathit{const}, \text{such that } \sigma(v) = \mathit{const}\}$\;
   }
   $\mathit{cnt} \longleftarrow 0$\;
   \While {$C \neq \emptyset$ \And $\mathit{cnt} < 20$} {
     \text{let $c \in C$ maximizes $F(R\prime, S\prime, c)$}\;
     $C \longleftarrow C/\{c\}$\;
     \If {$\mathrm{Test}(\langle p\prime[c/\texttt{abstc}], n\prime \rangle, \mathit{NegT}, \mathit{PosT})$} {
       \Return $\langle p\prime[c/\texttt{abstc}], n\prime \rangle$\;
     }
     $\mathit{cnt} \longleftarrow \mathit{cnt} + 1$\;
   }
 }
 \ElseIf {$p\prime$ contains \texttt{abstval}} {
   $C \longleftarrow \texttt{Variable} \cup \texttt{Int}$\;
   \For {$\langle I, O \rangle$ \In $\mathit{NegT}$} {
     $\langle O\prime, \_ , S \rangle \longleftarrow \mathrm{Exec}(\langle p\prime, n\prime \rangle, I, \epsilon)$\;
     $C \longleftarrow V(O\prime, O, S, C)$\;
   }
   \For {$\mathit{val}$ \In C} {
     \If {$\mathrm{Test}(\langle p\prime[\mathit{val}/\texttt{abstval}], n\prime \rangle, \mathit{NegT}, \mathit{PosT})$} {
       \Return $\langle p\prime[\mathit{val}/\texttt{abstval}], n\prime \rangle$\;
     }
   }
 }
 \ElseIf {$\mathrm{Test}(\langle p\prime, n\prime \rangle, \mathit{NegT}, \mathit{PosT})$} {
     \Return $\langle p\prime, n\prime \rangle$\;
 }
}
\Return $\emptyset$
\caption{Repair generation algorithm with condition synthesis}
\label{fig:repair}
\vspace{-4mm}
\end{algorithm}


\noindent \textbf{Condition Generation:}
The algorithm enumerates all conditions in the search space and 
evaluates each condition against the recorded condition values
(R$\prime$) and environments ($S\prime$). It counts the number
of recorded condition values that the condition matches. Our
current condition space is the set of all conditions of the
form \texttt{($v$ == $\mathit{const}$)} or \texttt{!($v$ == $\mathit{const}$)} 
such that $\exists \sigma \in S\prime .  \sigma(v) = \mathit{const}$. 
It is straightforward to extend this space to include comparison
operators $(<, \leq, \geq, >)$ and a larger set of logical expressions.
For our benchmark set of defects, the current {\name} condition space contains a remarkable
number of correct repairs, with extensions to this space delivering relatively
few additional correct repairs (see Section~\ref{sec:results:searchspace}).

$\mathrm{F(R\prime, S\prime, c)}$ in Figure~\ref{fig:repair} is an utility
function that counts the number of branch directions for the condition $c$ that
match the recorded abstract condition values $R\prime$ given the recorded
environments $S\prime$. See Figure~\ref{fig:exec-test-flip-f} for the
formal definition. The algorithm enumerates a configurable number (in our current
implementation, 20) of the top conditions that maximize
$F(R\prime, S\prime, c)$ (lines 27-33). The algorithm then validates the
transformed candidate program with the abstract condition replaced by the
generated condition $c$ (lines 31-32). $p[c/\texttt{abstc}]$ denotes the result
of replacing every occurrence of $\texttt{abstc}$ in $p$ with the condition
$c$.

Enumerating all conditions in the space is feasible because 
the overwhelming majority of the candidate 
transformed programs do not pass the target condition value search stage.
{\name} will therefore perform the condition generation stage very 
infrequently and only when there is some evidence that transforming
the target condition may deliver a correct repair. 
In our experiments, {\name} performs the condition generation stage
for less than 1\% of the candidate programs 
that contain an abstract condition (see Section~\ref{sec:designchoices}).

\noindent{\bf Staged Repair for Print Statements: } We augment the semantics to
support print statements with abstract expressions as shown as the fourth rule in
Figure~\ref{fig:semantic-abstc}. When such a print statement is executed, a
special token \texttt{abstval} is appended to the output sequence $O$ to
represent an undetermined value.

At the first stage, the algorithm executes the program with such abstract print
statements on each of the negative test cases (lines 35-38). The algorithm
compares the result output sequence $O\prime$ with the expected output sequence
$O$. This comparison uses the utility function $V(O\prime, O, S, C)$ to compute a set of
concrete values that, after replacing the abstract expression, enable the
repaired program to pass the test case. See Figure~\ref{fig:exec-test-flip-f}
for the formal definition of $V$. If the first stage succeeds, 
the second stage replaces the abstract expression with the computed concrete values and validates
the resulting repair (lines 39-41).

\if 0
\noindent{\bf Alternate Condition Synthesis Techniques:} It is straightforward to implement a
variety of different condition synthesis techniques. For example, it is possible
to synthesize complete replacements for conditions of if statements (instead of conjoining
or disjoining new conditions to existing conditions). The condition value search
would start with the sequence of branch directions at that if statement
with the original condition, then search for a sequence of branch directions
that would generate correct outputs
for all negative inputs. Condition generation would then work with the recorded
branch directions to deliver a new replacement condition. 

The effectiveness of condition value search in eliminating 
unpromising conditions enables the {\name} condition generation algorithm 
to simply enumerate and test all conditions in the condition search
space.  It is of course possible to apply arbitrarily sophisticated 
condition generation algorithms, for example by leveraging modern
solver technology~\cite{Nguyen:2013}. One issue is that there may be no condition 
that exactly matches the recorded sequences of environments and branch 
directions. Even if this occurs infrequently (as we would expect
in practice), requiring an exact match may eliminate otherwise correct repairs.  
An appropriate solver may therefore need to generate approximate solutions. 
\fi


\subsection{Extensions for C}
\label{sec:design:extensions}

\if 0
Clang contains a set of APIs for manipulating the AST tree of a parsed C
program, which enables {\name} to generate a repaired source code file without
dramatically changing the overall structure of the source code. Existing
program repair tools~\cite{LeGoues:2012, Qi:2014, Weimer:2013} often destroy
the structure of the original source by inlining all header files and renaming
all local variables in their generated repaired source code. Preserving the
existing source code structure helps developers understand and evaluate the
repair and promotes the future maintainability of the application. 
\fi

\noindent \textbf{C Program Support: } 
We have implemented {\name} in C++ using the clang compiler
front-end~\cite{clang}. % {\name} extends the algorithm to support C programs.
{\name} applies the transformation function separately to each function in a C
program. When {\name} performs variable replacement or condition synthesis, it
considers all variables (including local, global, and heap variables) that
appear in the transformed function. During condition generation, {\name} also
searches existing conditions $c$ that occur in the same enclosing compound
statement (in addition to conditions of the form \texttt{($v$ ==
$\mathit{const}$)} or \texttt{!($v$ == $\mathit{const}$)} described in
Section~\ref{sec:design:algo}).

When {\name} inserts control statements, {\name} generates repairs
that include \sourcecode{break},
\sourcecode{return}, and \sourcecode{goto} statements. When inserting
\sourcecode{return} statements, {\name} generates a repair to return each
constant value in the returned type that appeared in the enclosing function.
When inserting \sourcecode{goto} statements, {\name} generates a repair to jump
to each already defined label in the enclosing function. When {\name} inserts
initialization statements, {\name} generates repairs that call \sourcecode{memset()} to
initialize memory blocks.  When {\name} copies statements, {\name} generates
repairs that copy compound statements in addition to simple statements, as long as the
copied code can fit into the new context. {\name} also extends its staged
repair algorithm to constant string literals in C print statements (e.g.,
\sourcecode{printf()}). See our technical report~\cite{SPRTechReport} for implementation
details.

\if 0
To represent a abstract condition, {\name} inserts a function call
\sourcecode{abstract\_code()} into the modified condition. When {\name} tests a candidate
transformed program with abstract conditions, {\name} links the program with
its runtime library, which contains an implementation of
\sourcecode{abstract\_cond()}. The \sourcecode{abstract\_cond()} in the library
implements the semantics specified in Figure~\ref{fig:semantic-abstc}.
\fi

\noindent \textbf{Error Localizer:} 
The {\name} error localizer recompiles the given application with additional
instrumentation. It inserts a call back before each statement in the source
code to record a positive counter value as the timestamp of the statement
execution. {\name} then invokes the recompiled application on all test cases
and produces a prioritized list that contains target statements to modify based
on the recorded timestamp values. {\name} prioritizes statements that 1) 
execute on more negative test cases, 2) execute on fewer positive
test cases, and 3) execute later on negative test
cases executions. Our technical report~\cite{SPRTechReport} presents the error localization
algorithm.


\if 0
{\name} then invokes the recompiled application on all
the positive and negative test cases. 

For a statement $s$ and a test case $i$, $r(s, i)$ is the recorded execution
timestamp that corresponds to the last timestamp from an execution of the statement
$s$ when the application runs with the test case $i$. If the statement $s$ is
not executed at all when the application runs with the test case $i$, then
$r(s, i) = 0$. 

We use the notation $\mathrm{NegT}$ for the set of negative test cases and 
$\mathrm{PosT}$ for the set of positive test cases. {\name} computes three
scores $a(s)$, $b(s)$, $c(s)$ for each statement $s$:
\begin{displaymath}
\begin{array}{l}
a(s)= \left\vert\; \left\{i \; \mid \; r(s, i) \neq 0, \, i  \in \mathrm{NegT}\right\} \; \right\vert \\
b(s)= \left\vert\; \left\{i \; \mid \; r(s, i) = 0, \, i \in \mathrm{PosT}\right\} \; \right\vert \\
c(s)= \Sigma_{i \in \mathrm{NegT}} r(s, i) \\
\end{array}
\end{displaymath}

A statement $s_1$ has higher priority than a statement $s_2$ if $\mathrm{prior}(s_1, s_2) = 1$,
where $\mathrm{prior}$ is defined as:
\begin{displaymath}
prior(s_1, s_2) = \left\{
\begin{array}{ll}
1  & a(s_1) > a(s_2) \\
1  & a(s_1) = a(s_2), b(s_1) > b(s_2) \\
\multirow{2}{*}{1}  & a(s_1) = a(s_2), b(s_1) = b(s_2), \\
       & c(s_1) > c(s_2) \\
0  & \text{otherwise}
\end{array}
\right. 
\end{displaymath}

Intuitively, {\name} prioritizes statements that 1) are executed with more negative
test cases, 2) are executed with fewer positive test cases, and 3)
are executed later during executions with negative test cases.

{\name} runs the above error localization algorithm over the whole application
including all of its C source files. If the user specifies a source file to
repair, {\name} computes the intersection of the top 5000 statements in the
whole application with the statements in the specified source code file.
PCR uses the statements in this intersection as the identified statements to repair.
Unlike GenProg~\cite{LeGoues:2012} and AE~\cite{Weimer:2013}, {\name} can also operate
completely automatically. If the user does not specify any such source file,
{\name} identifies the top 200 statements in the whole application (potentially
from different source files) as the potential modification targets.

The {\name} error localizer also ranks if statements based on the statements
inside their then and else clauses. Specifically, it gives an if statement
the rank of the highest ranking statement in its then or else clauses. 
The rationale is that changing the condition of these enclosing if statement will
control the execution of the identified statement and therefore may repair the
program.
\fi

\noindent \textbf{Repair Test Order: } 
{\name} validates the generated
candidate repairs one by one (line 1 in Figure~\ref{fig:repair}). {\name}
prioritizes the generated patches as follows:
\begin{enumerate} % \itemsep 0pt \parskip 0pt
\item {\name} first tests repairs that change only a branch condition (e.g., tighten and
loosen a condition).
\item {\name} tests repairs that insert an if-statement before a statement $s$,
where $s$ is the first statement of a compound statement (i.e., C code block).
\item {\name} tests repairs that insert an if-guard around a statement $s$.
\item {\name} tests repairs with abstract print statements.
\item {\name} tests repairs that insert a memory initialization.
\item {\name} tests repairs that insert an if-statement before a statement $s$,
where $s$ is not the first statement of a compound statement.
\sloppypar{
\item {\name} tests repairs a) that replace a statement or b) that insert a non-if 
statement (i.e., generated by $\mathrm{M_{\text{CpRep}}}$) before a statement $s$ 
where $s$ is the first statement of a compound statement.
}
\item {\name} finally tests the remaining repairs. 
\end{enumerate}

\if 0
Intuitively, {\name} prioritizes repairs that contain conditionals. With
abstract conditions that {\name} later synthesizes, each condition value
search stands in for multiple potential repairs.  {\name} also prioritizes repairs that
insert a statement before the first statement of a compound statement (i.e., a
code block), because inserting statements at other locations is often
semantically equivalent to such repairs.
\fi

If two repairs have the same tier in the previous list, their validation order is
determined by the rank of the two corresponding original statements (which the two
repairs modify) in the list returned by the error localizer. 

\if 0
\noindent {\textbf{Optimizations:}} {\name} uses a set of optimizations to
speed up the candidate program compilation and testing. {\name} also detects
code duplicates in the program and appropriately propagates the generated
repair to each code duplicate if neccessary. See our technical
report~\cite{SPRTechReport}.
\fi

\if 0
\noindent {\textbf{Batched Compilation:}} When {\name} tests candidate repairs,
compilations of the repaired application may become the performance bottleneck
for {\name}. 
%In our experiments, it may take up to one minutes to
%recompile the repaired source file and to relink the repaired application. 
To reduce the time cost of compilations, {\name} merges similar candidate
repairs into a single combined repair with a branch statement. A global integer
environment variable controls the branch statement, so that the batched repair
will be equivalent to each individual candidate repair, when the environment
variable takes a corresponding constant value. {\name} therefore only needs to
recompile the merged repair once to test each of the individual candidate repairs.

\noindent {\textbf{Test Case Evaluation Order: }} {\name} always first tests
each candidate repair with the negative test cases. Empirically, negative test cases
tend to eliminate invalid repairs more effectively than positive test cases.
Furthermore, whenever a positive test case eliminates a candidate repair, {\name}
will record this positive test case and prioritize this test case for the
future candidate repair evaluation.

\noindent {\textbf{Repairs for Code Duplicates: }} Programs
often contain duplicate or similar source code, often caused, for example, by the
use of macros or code copy/paste during application development. {\name}
detects such duplicates in the source code. When {\name} generates repairs
that modify one of the duplicates, it also generates
additional repairs that propagate the modification to the other duplicates.
\fi

\if 0
\subsection{Implementation}

We have implemented {\name} in C++ using the clang compiler
front-end~\cite{clang}. We choose clang because it has a AST tree
interface that contains APIs that support source code rewrites. 
This enables {\name} to generate a patched source code file without
dramatically changing the overall structure of the source code. 
Existing program repair tools~\cite{LeGoues:2012, Qi:2014, Weimer:2013} often 
destroy the structure of the original source by inlining
all header files and renaming all local variables in their generated patched
source code. Preserving the existing source code structure helps developers
understand and evaluate the patch and promotes the future maintainability of the application.
\fi


==> figs/tab-comp-nophp-3.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Search Space}} & \multirow{2}{*}{\scriptsize \textbf{SPR}} & \multirow{2}{*}{\scriptsize \textbf{Prophet}} & \textbf{\scriptsize Random} & \textbf{\scriptsize Random} \\
& & & \textbf{\scriptsize (SPR)} & \textbf{\scriptsize (Prophet)} \\
\hline
100+No & 22.0 \ 2.0 & 16.0 \ 4.0 & 23.3 \ 0.7 & 23.3 \ 0.7 \\
\hline
100+CExt & 22.0 \ 1.0 & 18.0 \ 3.0 & 23.4 \ 0.6 & 23.4 \ 0.6 \\
\hline
100+RExt & 22.0 \ 2.0 & 16.0 \ 4.0 & 23.3 \ 0.7 & 23.3 \ 0.7 \\
\hline
100+RExt+CExt & 22.0 \ 1.0 & 18.0 \ 3.0 & 23.4 \ 0.6 & 23.4 \ 0.6 \\
\hline
200+No & 23.0 \ 3.0 & 17.0 \ 5.0 & 24.8 \ 1.5 & 25.0 \ 1.4 \\
\hline
200+CExt & 23.0 \ 2.0 & 19.0 \ 4.0 & 25.1 \ 1.2 & 25.1 \ 1.2 \\
\hline
200+RExt & 23.0 \ 3.0 & 17.0 \ 5.0 & 24.7 \ 1.3 & 24.7 \ 1.3 \\
\hline
200+RExt+CExt & 23.0 \ 2.0 & 19.0 \ 4.0 & 24.8 \ 1.2 & 24.8 \ 1.2 \\
\hline
300+No & 25.0 \ 2.0 & 19.0 \ 4.0 & 26.3 \ 0.7 & 26.0 \ 0.9 \\
\hline
300+CExt & 25.0 \ 1.0 & 21.0 \ 3.0 & 26.6 \ 0.4 & 26.5 \ 0.5 \\
\hline
300+RExt & 25.0 \ 2.0 & 19.0 \ 4.0 & 26.6 \ 0.4 & 26.3 \ 0.7 \\
\hline
300+RExt+CExt & 25.0 \ 1.0 & 21.0 \ 3.0 & 26.7 \ 0.3 & 26.6 \ 0.4 \\
\hline
2000+No & 23.0 \ 3.0 & 19.0 \ 4.0 & 26.6 \ 0.4 & 26.1 \ 0.9 \\
\hline
2000+CExt & 23.0 \ 2.0 & 21.0 \ 3.0 & 26.8 \ 0.2 & 26.5 \ 0.5 \\
\hline
2000+RExt & 23.0 \ 3.0 & 20.0 \ 4.0 & 26.2 \ 0.8 & 26.2 \ 0.8 \\
\hline
2000+RExt+CExt & 23.0 \ 2.0 & 22.0 \ 3.0 & 26.4 \ 0.6 & 26.6 \ 0.4 \\
\hline
\end{tabular}


==> figs/tab-comp-nophp-5.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Search Space}} & \multirow{2}{*}{\scriptsize \textbf{SPR}} & \multirow{2}{*}{\scriptsize \textbf{Prophet}} & \textbf{\scriptsize Random} & \textbf{\scriptsize Random} \\
& & & \textbf{\scriptsize (SPR)} & \textbf{\scriptsize (Prophet)} \\
\hline
100+No & 32.0 \ 3.0 & 23.0 \ 4.0 & 36.5 \ 1.2 & 36.5 \ 1.2 \\
\hline
100+CExt & 35.0 \ 2.0 & 28.0 \ 3.0 & 38.0 \ 1.0 & 38.0 \ 1.0 \\
\hline
100+RExt & 32.0 \ 3.0 & 23.0 \ 4.0 & 36.6 \ 1.2 & 36.6 \ 1.2 \\
\hline
100+RExt+CExt & 35.0 \ 2.0 & 28.0 \ 3.0 & 38.0 \ 1.0 & 38.0 \ 1.0 \\
\hline
200+No & 34.0 \ 4.0 & 25.0 \ 5.0 & 39.6 \ 1.9 & 40.2 \ 1.6 \\
\hline
200+CExt & 36.0 \ 3.0 & 29.0 \ 4.0 & 40.6 \ 1.4 & 40.6 \ 1.4 \\
\hline
200+RExt & 34.0 \ 4.0 & 25.0 \ 5.0 & 39.9 \ 1.5 & 39.9 \ 1.6 \\
\hline
200+RExt+CExt & 36.0 \ 3.0 & 29.0 \ 4.0 & 40.3 \ 1.4 & 40.3 \ 1.4 \\
\hline
300+No & 38.0 \ 3.0 & 29.0 \ 4.0 & 42.6 \ 1.1 & 41.9 \ 1.4 \\
\hline
300+CExt & 40.0 \ 2.0 & 33.0 \ 3.0 & 43.6 \ 0.7 & 43.4 \ 0.8 \\
\hline
300+RExt & 38.0 \ 3.0 & 29.0 \ 4.0 & 43.5 \ 0.7 & 42.8 \ 1.1 \\
\hline
300+RExt+CExt & 40.0 \ 2.0 & 33.0 \ 3.0 & 43.9 \ 0.5 & 43.8 \ 0.6 \\
\hline
2000+No & 35.0 \ 3.0 & 29.0 \ 4.0 & 43.6 \ 0.7 & 42.1 \ 1.4 \\
\hline
2000+CExt & 37.0 \ 2.0 & 33.0 \ 3.0 & 44.3 \ 0.4 & 43.3 \ 0.8 \\
\hline
2000+RExt & 35.0 \ 3.0 & 30.0 \ 4.0 & 42.3 \ 1.4 & 42.2 \ 1.4 \\
\hline
2000+RExt+CExt & 37.0 \ 2.0 & 34.0 \ 3.0 & 42.9 \ 1.0 & 43.7 \ 0.6 \\
\hline
\end{tabular}


==> figs/tab-comp-php-3.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Search Space}} & \multirow{2}{*}{\scriptsize \textbf{SPR}} & \multirow{2}{*}{\scriptsize \textbf{Prophet}} & \textbf{\scriptsize Random} & \textbf{\scriptsize Random} \\
& & & \textbf{\scriptsize (SPR)} & \textbf{\scriptsize (Prophet)} \\
\hline
100+No & 17.0 \ 8.0 & 17.0 \ 8.0 & 20.7 \ 6.8 & 20.6 \ 6.9 \\
\hline
100+CExt & 20.0 \ 8.0 & 23.0 \ 7.0 & 25.4 \ 5.6 & 25.5 \ 5.5 \\
\hline
100+RExt & 20.0 \ 9.0 & 18.0 \ 9.0 & 23.2 \ 7.3 & 23.4 \ 7.1 \\
\hline
100+RExt+CExt & 20.0 \ 8.0 & 23.0 \ 7.0 & 25.5 \ 5.5 & 25.4 \ 5.6 \\
\hline
200+No & 18.0 \ 9.0 & 19.0 \ 10.0 & 22.4 \ 7.8 & 24.7 \ 8.5 \\
\hline
200+CExt & 18.0 \ 9.0 & 24.0 \ 8.0 & 24.2 \ 6.5 & 27.1 \ 6.6 \\
\hline
200+RExt & 18.0 \ 9.0 & 19.0 \ 10.0 & 22.4 \ 7.8 & 24.9 \ 8.2 \\
\hline
200+RExt+CExt & 18.0 \ 9.0 & 24.0 \ 8.0 & 24.2 \ 6.5 & 27.1 \ 6.6 \\
\hline
300+No & 19.0 \ 8.0 & 19.0 \ 10.0 & 22.9 \ 7.2 & 25.8 \ 8.4 \\
\hline
300+CExt & 19.0 \ 8.0 & 24.0 \ 8.0 & 25.2 \ 5.4 & 28.8 \ 5.9 \\
\hline
300+RExt & 19.0 \ 8.0 & 19.0 \ 10.0 & 22.9 \ 7.2 & 25.9 \ 8.3 \\
\hline
300+RExt+CExt & 19.0 \ 8.0 & 24.0 \ 8.0 & 25.2 \ 5.4 & 28.5 \ 6.2 \\
\hline
2000+No & 7.0 \ 5.0 & 13.0 \ 7.0 & 10.8 \ 3.7 & 17.5 \ 5.5 \\
\hline
2000+CExt & 7.0 \ 5.0 & 15.0 \ 5.0 & 12.7 \ 2.3 & 17.7 \ 3.3 \\
\hline
2000+RExt & 9.0 \ 5.0 & 10.0 \ 6.0 & 12.8 \ 3.7 & 14.5 \ 4.5 \\
\hline
2000+RExt+CExt & 7.0 \ 5.0 & 13.0 \ 5.0 & 12.7 \ 2.3 & 17.6 \ 2.4 \\
\hline
\end{tabular}


==> figs/tab-comp-php-5.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Search Space}} & \multirow{2}{*}{\scriptsize \textbf{SPR}} & \multirow{2}{*}{\scriptsize \textbf{Prophet}} & \textbf{\scriptsize Random} & \textbf{\scriptsize Random} \\
& & & \textbf{\scriptsize (SPR)} & \textbf{\scriptsize (Prophet)} \\
\hline
100+No & 23.0 \ 8.0 & 23.0 \ 8.0 & 28.9 \ 7.2 & 28.6 \ 7.4 \\
\hline
100+CExt & 28.0 \ 8.0 & 33.0 \ 7.0 & 38.1 \ 5.9 & 38.2 \ 5.9 \\
\hline
100+RExt & 26.0 \ 9.0 & 24.0 \ 9.0 & 32.2 \ 7.9 & 32.9 \ 7.8 \\
\hline
100+RExt+CExt & 28.0 \ 8.0 & 33.0 \ 7.0 & 38.2 \ 5.9 & 38.2 \ 5.9 \\
\hline
200+No & 24.0 \ 9.0 & 25.0 \ 10.0 & 30.7 \ 8.2 & 33.3 \ 9.4 \\
\hline
200+CExt & 24.0 \ 9.0 & 34.0 \ 8.0 & 35.1 \ 6.8 & 39.8 \ 6.9 \\
\hline
200+RExt & 24.0 \ 9.0 & 25.0 \ 10.0 & 30.7 \ 8.2 & 34.1 \ 9.0 \\
\hline
200+RExt+CExt & 24.0 \ 9.0 & 34.0 \ 8.0 & 35.1 \ 6.8 & 39.7 \ 7.0 \\
\hline
300+No & 24.0 \ 9.0 & 25.0 \ 10.0 & 30.2 \ 7.7 & 34.3 \ 9.4 \\
\hline
300+CExt & 24.0 \ 9.0 & 34.0 \ 8.0 & 36.2 \ 5.7 & 42.8 \ 6.4 \\
\hline
300+RExt & 24.0 \ 9.0 & 25.0 \ 10.0 & 30.2 \ 7.7 & 34.6 \ 9.2 \\
\hline
300+RExt+CExt & 24.0 \ 9.0 & 34.0 \ 8.0 & 36.3 \ 5.7 & 41.6 \ 7.0 \\
\hline
2000+No & 7.0 \ 5.0 & 17.0 \ 7.0 & 13.1 \ 4.2 & 24.3 \ 5.8 \\
\hline
2000+CExt & 7.0 \ 5.0 & 21.0 \ 5.0 & 18.0 \ 2.5 & 27.0 \ 3.5 \\
\hline
2000+RExt & 9.0 \ 5.0 & 12.0 \ 6.0 & 15.1 \ 4.2 & 19.3 \ 4.8 \\
\hline
2000+RExt+CExt & 7.0 \ 5.0 & 17.0 \ 5.0 & 18.1 \ 2.5 & 26.8 \ 2.6 \\
\hline
\end{tabular}


==> figs/tab-comparison-nophp.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Search Space}} & \multirow{2}{*}{\scriptsize \textbf{SPR}} & \multirow{2}{*}{\scriptsize \textbf{Prophet}} & \textbf{\scriptsize Random} & \textbf{\scriptsize Random} \\
& & & \textbf{\scriptsize (SPR)} & \textbf{\scriptsize (Prophet)} \\
\hline
100+No & 12.5\% & 50.0\% & 3.1\% & 3.1\% \\
\hline
100+CExt & 12.5\% & 25.0\% & 2.5\% & 2.5\% \\
\hline
100+RExt & 12.5\% & 50.0\% & 3.1\% & 3.1\% \\
\hline
100+RExt+CExt & 12.5\% & 25.0\% & 2.5\% & 2.5\% \\
\hline
200+No & 22.2\% & 55.6\% & 9.4\% & 8.7\% \\
\hline
200+CExt & 22.2\% & 33.3\% & 8.6\% & 8.7\% \\
\hline
200+RExt & 22.2\% & 44.4\% & 12.3\% & 12.4\% \\
\hline
200+RExt+CExt & 22.2\% & 33.3\% & 12.3\% & 12.4\% \\
\hline
300+No & 11.1\% & 44.4\% & 2.7\% & 3.8\% \\
\hline
300+CExt & 11.1\% & 33.3\% & 2.0\% & 2.3\% \\
\hline
300+RExt & 11.1\% & 33.3\% & 1.6\% & 3.8\% \\
\hline
300+RExt+CExt & 11.1\% & 33.3\% & 1.6\% & 2.4\% \\
\hline
2000+No & 11.1\% & 33.3\% & 1.5\% & 3.3\% \\
\hline
2000+CExt & 11.1\% & 22.2\% & 1.2\% & 2.4\% \\
\hline
2000+RExt & 11.1\% & 22.2\% & 3.0\% & 4.0\% \\
\hline
2000+RExt+CExt & 11.1\% & 22.2\% & 2.7\% & 2.6\% \\
\hline
\end{tabular}


==> figs/tab-comparison-php.tex <==
\begin{tabular}{|l|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Search Space}} & \multirow{2}{*}{\scriptsize \textbf{SPR}} & \multirow{2}{*}{\scriptsize \textbf{Prophet}} & \textbf{\scriptsize Random} & \textbf{\scriptsize Random} \\
& & & \textbf{\scriptsize (SPR)} & \textbf{\scriptsize (Prophet)} \\
\hline
100+No & 72.7\% & 72.7\% & 52.6\% & 52.8\% \\
\hline
100+CExt & 50.0\% & 50.0\% & 43.2\% & 43.2\% \\
\hline
100+RExt & 66.7\% & 75.0\% & 49.4\% & 48.9\% \\
\hline
100+RExt+CExt & 50.0\% & 50.0\% & 43.2\% & 43.2\% \\
\hline
200+No & 75.0\% & 76.9\% & 52.2\% & 50.1\% \\
\hline
200+CExt & 58.3\% & 53.8\% & 47.1\% & 43.8\% \\
\hline
200+RExt & 75.0\% & 76.9\% & 52.2\% & 49.2\% \\
\hline
200+RExt+CExt & 58.3\% & 53.8\% & 47.2\% & 43.8\% \\
\hline
300+No & 66.7\% & 76.9\% & 45.1\% & 44.7\% \\
\hline
300+CExt & 58.3\% & 53.8\% & 38.7\% & 36.8\% \\
\hline
300+RExt & 66.7\% & 76.9\% & 45.1\% & 44.2\% \\
\hline
300+RExt+CExt & 58.3\% & 53.8\% & 38.7\% & 37.7\% \\
\hline
2000+No & 57.1\% & 66.7\% & 39.2\% & 46.5\% \\
\hline
2000+CExt & 42.9\% & 37.5\% & 30.0\% & 38.8\% \\
\hline
2000+RExt & 50.0\% & 62.5\% & 34.3\% & 39.8\% \\
\hline
2000+RExt+CExt & 28.6\% & 25.0\% & 29.9\% & 26.5\% \\
\hline
\end{tabular}


==> paper_related.tex <==
\section{Related Work}
\label{sec:related_work}

\noindent{\bf ClearView:} 
ClearView is a generate-and-validate system that observes normal executions to
learn invariants that characterize safe behavior~\cite{Perkins:2009}. It deploys
monitors that detect crashes, illegal control transfers and out of bounds write
defects. In response, it selects a nearby invariant that the input that
triggered the defect violates, and generates patches that take a repair action
to enforce the invariant. 

A Red Team evaluation found that ClearView was able to automatically generate patches
that eliminate 9 of 10 targeted Firefox vulnerabilities~\cite{Perkins:2009},
with each defect eliminated after the generation of at most three patches. 
We attribute the density with which successful patches appear in the ClearView search 
space, in part, to the fact that ClearView leverages the learned invariant
information to focus the search on successful patches and does not rely 
solely on the validation test suite. 

\noindent{\bf Kali:} Kali is a generate-and-validate system that 
deploys a simple strategy --- it simply removes functionality. 
Although Kali is obviously not
intended to correctly repair a reasonable subset of the defects that occur
in practice, it is nevertheless at least
as effective in practice 
as previous strategies that aspire to 
repair a broad class of defects~\cite{Kali}. 

These results are consistent with the results presented in this paper, highlight the
inadequacy of current test suites to successfully identify incorrect patches,
and identify one prominent source of the relatively many plausible but incorrect patches 
that occur in current patch search spaces. 

A recent paper ~\cite{NOPOLTR} 
evaluates Kali remove statement patches,
GenProg patches,
and NOPOL~\cite{DeMarco:2014} patches for 224
defects in the Defects4J dataset~\cite{Defects4J}. The results
are, in general, consistent with our results in this paper. 
Out of 42 manually analyzed plausible patches, the analysis indicates that only 8
patches are undoubtedly correct.

\noindent{\bf GenProg, AE, and RSRepair:} GenProg~\cite{LeGoues:2012}, AE~\cite{Weimer:2013}, 
and RSRepair~\cite{Qi:2014} were all evaluated on (for RSRepair, a subset of)
the same benchmark set that we use
in this paper to evaluate the SPR and Prophet search spaces. The evaluations
focus on plausible patches with no attempt to determine whether the patches
are correct or not.  Unfortunately, the presented evaluations of these systems suffer 
from the fact that the testing
infrastructure used to validate the candidate patches contains errors that
cause the systems to incorrectly accept 
implausible patches that do not even pass all of the test
cases in the validation test suite~\cite{Kali}. 

A subsequent study corrects these errors and
sheds more light on the subject~\cite{Kali}. This 
study found that 1) the systems generate correct patches for only 2 (GenProg, RSRepair)
or 3 (AE) of the 105 benchmark defects/functionality changes in this
benchmark set, 2) the systems generate plausible but
incorrect patches for 16 (GenProg), 8 (RSRepair), and 24 (AE) 
defects/functionality changes, and 
3) the majority of the plausible patches, including all correct patches,
are equivalent to a single modification that deletes functionality. 
Moreover, the correct SPR and Prophet patches for these defects lie outside the
GenProg, AE, and RSRepair search space (suggesting that these systems will
never be able to generate a correct patch for these defects)~\cite{SPR}.

Moreover, only 5 of the 110 plausible GenProg patches are correct,
only 4 of the analyzed plausible 44 RSRepair patches are correct, and only 3 of the 27
plausible AE patches are correct~\cite{Kali}. These results indicate
that the GenProg, AE, and RSRepair search space, while containing fewer correct
and plausible patches than the richer SPR and Prophet search
spaces~\cite{SPR,Prophet}, still exhibits the basic pattern of sparse correct
patches and more abundant plausible but incorrect patches.

A subsequent study of GenProg and RSRepair (under the name TrpAutoRepair) on small student programs
provides further support for this hypothesis~\cite{Overfitting}. The results indicate that patches
validated on one test suite typically fail to generalize to produce correct results
on other test suites. 

RSRepair uses random search; previous
research found that the GenProg genetic search algorithm 
performs no better than random search on a subset of the benchmarks~\cite{Qi:2014}. 
Systems (such as GenProg) that perform no better than random will need to 
incorporate additional sources of information other than the validation test suite
if they are to successfully generate correct patches in the presence
of current relatively weak test suites.\footnote{
Of course, if the patch space does not contain correct patches,
stronger test suites will prevent the system from generating
any patches at all. This is the case for GenProg ---
at most two additional test cases per defect completely disable GenProg's
ability to produce any patch at all except the five correct patches
in its search space~\cite{Kali}.
}

\noindent {\bf PAR:}
PAR is based on a set of predefined human-provided patch templates~\cite{Kim:2013}.
We are unable to directly compare PAR with other
systems because, despite repeated requests to the authors of the PAR paper over
the course of 11 months, the authors never provided us with the patches that
PAR was reported to have generated~\cite{Kim:2013} or the necessary materials to
would have enabled us to reproduce the PAR experiments.

\sloppypar{
The PAR search space (with the eight templates in the PAR paper~\cite{Kim:2013}) is in fact a subset
of the SPR and Prophet search space. Monperrus found that PAR fixes the
majority of its benchmark defects with only two templates (``Null Pointer
Checker'' and ``Condition Expression
Adder/Remover/Replacer'')~\cite{Monperrus:2014}.
}

\noindent{\bf NOPOL:}
NOPOL~\cite{DeMarco:2014, NOPOLTR} is an automatic repair tool focusing on branch
conditions. It identifies branch statement directions that can pass negative
test cases and then uses SMT solvers to generate repairs for the branch
condition. 

\noindent{\bf Data Structure Repair:} Data structure repair enables applications
to recover from data structure corruption errors~\cite{DemskyR03,DemskyR06}. It
enforces a data structure consistency specification. This specification
can be provided by a developer or automatically inferred from correct
program executions~\cite{DemskyEGMPR06}.

In general, there are multiple repaired data structures that satisfy the
consistency specification.  Data structure repair operates over search space 
generated by a set of repair operations to generate a repaired data structure
that is heuristically close to the original unrepaired data structure. The
goal is not to obtain a hypothetical data structure, but instead a consistent data
structure that enables acceptable continued execution. 


%Monperrus found that PAR fixes the majority of its
%benchmark defects with only two templates (``Null Pointer Checker'' and
%``Condition Expression Adder/Remover/Replacer'')~\cite{Monperrus:2014}. 

\noindent{\bf SemFix and MintHint:}
SemFix~\cite{Nguyen:2013} and MintHint~\cite{Kaleeswaran:2014} replace the
faulty expression with a symbolic value and use symbolic execution
techniques~\cite{KLEE} to find a replacement expression that
enables the program to pass all test cases. SemFix and MintHint are 
evaluated only on applications with less than 10000 lines of code. 
In addition, these techniques cannot generate fixes for statements
with side effects. 

\noindent{\bf Defect Repair via Q\&A Sites: } Gao et. al.~\cite{QingGaoASE15}
propose to repair recurring defects by analyzing Q\&A sites such as Stack
Overflow. The proposed technique locates the relevant Q\&A page for a recurring
defect via a search engine query, extracts code snippets from the page, and
renames variables in the extracted code snippets to generate patches. This
technique addresses the weak test suite problem with the additional information
collected from the Q\&A sites, but it requires the existence of exact defect
repair logic on Q\&A pages.

\noindent{\bf AutoFixE: }
AutoFix-E~\cite{AutoFix-E, AutoFixETSE} operates with a set of fix schemas to repair Eiffel
programs with human-supplied specifications called contracts. 

\noindent{\bf Characteristics of Human Patches:}
Barr et al.~\cite{Barr:2014} found that 
10\% of commits to a set of codebases can be completely constructed from existing code.  
Martinez et. al.~\cite{Martinez:2014} found that 3-17\% of the commits can be
synthesized from existing lines of code. 
Zhong and Su systematically analyzed more than
9000 real world bug fixes and studied several research questions including how
many locations each bug fix modifies and what modification operators are
essential for bug fixing~\cite{Zhong:2015}. 

% Martinez and Monperrus manually mined previous
% human patches and suggest that if a patch generation system works with a
% non-uniform probabilistic model, the system would find plausible patches
% faster~\cite{MiningRepairModel}. In contrast, Prophet~\cite{Prophet}
% automatically learns a probabilistic model from past successful patches.
% Prophet is the first patch generation system to operate with such a learned
% model to identify correct patches.

%\noindent{\bf Debroy and Wong:}
%Debroy and Wong~\cite{Debroy:2010} present a transformation-based patch generation
%technique. This technique either replaces an arithmetic operator with another
%operator or negates a condition. In contrast, {\name} uses more sophisticated
%and effective transformations and search algorithms. None of the correct
%repairs in {\name}'s search space for the 19 defects are within the Debroy and
%Wong search space. 


%\noindent{\bf Deductive Program Repair: }
%Deductive Program Repair formalizes the program repair problem as a program
%synthesis problem, using the original defective program as a
%hint~\cite{DeductiveProgramRepair}. It replaces the expression to repair with a
%synthesis hole and uses a counterexample-driven synthesis algorithm to find a
%patch that satisfies a formal specification. 

\sloppypar{
\noindent{\bf Domain Specific Repair Generation: }
Other program repair systems include VEJOVIS~\cite{Ocariza:2014} and Gopinath
et al.~\cite{Gopinath:2014}, which applies domain specific techniques to repair
DOM-related faults in JavaScript and selection statements in database programs
respectively. 
}

\noindent{\bf Dynamic Repair Techniques:} Researchers have developed
dynamic techniques for repairing memory errors~\cite{Rinard:2004}, 
null pointer dereference and divide by zero errors~\cite{Long:2014},
infinite loops~\cite{Carbin:2011,Kling:2012}, memory leaks~\cite{NguyenR07},
and corrupt data structures~\cite{DemskyR03,DemskyR06,DemskyEGMPR06}.

\noindent{\bf Self-Stabilizing Java:} Self-Stabilizing Java uses a type system
to ensure that the impact of any errors are eventually flushed from the
system, returning the system back to a consistent state~\cite{EomD12}.

\noindent{\bf Task Skipping and Loop Perforation:} 
Task skipping~\cite{Rinard06,Rinard07} discards task executions
and loop perforation~\cite{sidiroglou11} discards loop iterations. 
The result is a generated search space of programs with varying
performance and accuracy properties, some of which may be more
desirable than the original.  
In addition to enabling programs to survive tasks or loop iterations 
that trigger otherwise fatal errors, task skipping and loop perforation
can also improve performance. 

\noindent \textbf{CodePhage:}
Horizontal code transfer automatically locates correct code in one application,
then transfers that code into another application~\cite{Sidiroglou-Douskos15}.
This technique has been applied to eliminate otherwise fatal integer overflow,
buffer overflow, and divide by zero errors and shows enormous potential for
leveraging the combined talents and labor of software development efforts
worldwide. 



==> pygdef.tex <==
\usepackage{fancyvrb}
\usepackage{color}
\usepackage[latin1]{inputenc}



\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother

